Recurrent Relational Networks

This paper is concerned with learning to solve tasks that require a chain of interdependent steps of relational inference, like answering complex questions about the relationships between objects, or solving puzzles where the smaller elements of a solution mutually constrain each other. We introduce the recurrent relational network, a general purpose module that operates on a graph representation of objects. As a generalization of Santoro et al. [2017]'s relational network, it can augment any neural network model with the capacity to do many-step relational reasoning. We achieve state of the art results on the bAbI textual question-answering dataset with the recurrent relational network, consistently solving 20/20 tasks. As bAbI is not particularly challenging from a relational reasoning point of view, we introduce Pretty-CLEVR, a new diagnostic dataset for relational reasoning. In the Pretty-CLEVR set-up, we can vary the question to control for the number of relational reasoning steps that are required to obtain the answer. Using Pretty-CLEVR, we probe the limitations of multi-layer perceptrons, relational and recurrent relational networks. Finally, we show how recurrent relational networks can learn to solve Sudoku puzzles from supervised training data, a challenging task requiring upwards of 64 steps of relational reasoning. We achieve state-of-the-art results amongst comparable methods by solving 96.6% of the hardest Sudoku puzzles.

==> scratch-pad.tex <==
Many real life problems require relational reasoning in order to be solved. Consider understanding the simple sentence, e.g. "The police officer shot the burglar with the gun", which require reasoning about the people and items involved to infer the most likely meaning and resolve the ambiguity.
\emph{UP: a more politically neutral sentence?}
Or consider playing chess in which each piece affects each other piece and estimating the value of a move requires understanding how the pieces will likely affect each other over several turns ahead.
\emph{UP: If chess is not an example in the results, one should pick an example that fits the theme of the results. Call the opening example PROBLEM A}

Symbolic approaches to solving such problems are considered the traditional approach. This approach generally require defining each symbol and how it relates to each other symbol by hand.
\emph{UP: here, we don't yet know what symbols are...}
Given these definitions powerful algorithms such as search or constrained optimization can be employed and are in general very efficient.
\emph{UP: it's important that the story here ties in with your opening example. The reader can only think of one thing at a time, and you have to keep the telling of the story around that "one thing"}
However defining and recognizing symbols in the messy world of raw sensor inputs is often very hard.
\emph{UP: above, we have discrete alphabet of symbols. Is that different from what you propose below?}
For instance how do you define a car in pixel space? or the meaning of the word "shot"? As such the traditional approach has mostly been limited to more abstract cases where you can clearly and easily define the symbols \emph{UP like in which concrete example?}.

\emph{UP: I think the opening story line will be much more impactful if you contrast only two worlds, a traditional one (with one example) and one example where RRNs would help.}

Machine learning in general and deep learning in particular excel at messy real world sensor data
\emph{example of sensor data. should be the same as your opening "problem statement" example.}
however and have had great success at learning to recognize symbols in a wide range of raw inputs and domains.
\emph{UP it might help to be specific. what symbol? which raw input?}
But, whereas the traditional approach is weak at recognizing symbols but powerful at reasoning about them, for deep learning it is the other way around and many state-of-the-art deep learning approaches struggle with even simple relational reasoning \cite{santoro2017simple} TODO more cites.

\emph{UP. Here, you might want to make it clear that santoro's work and data sets are a step towards PROBLEM A, but is not sufficient.}
Recently \citet{santoro2017simple} took a step towards combining the best of both worlds using a simple and general approach. They propose to couple a deep learning perceptual front-end with a neural network relational reasoning module and train the joint model end-to-end. It is a compelling approach and they obtain super-human performance on the visual
question answering (QA)
dataset CLEVR, as well as good results on a BaBi, a set of textual reasoning tasks.

However, the complexity of the relational reasoning required in the datasets they use for evaluation is limited. The visual QA dataset CLEVR consists of images of 3D rendered objects with accompanying questions, e.g. "What is the color of the box left of the big cylinder" \cite{johnson2016clevr}. The number of reasoning steps required to produce an answer is never more than three. BaBi is a textual QA dataset by Facebook widely used in the deep learning literature \cite{weston2015towards}. It consists of 20 question-answering tasks that are designed to test various minimum requirements of reasoning. Again, the number of steps of relational reasoning required is never more than three.

\emph{This (above) is your selling point. I would put this paragraph much earlier, to ensure that the reader understands that the state of the art is 3 steps.}

Since we have plenty of evidence that deep learning models are powerful perceptual front-ends,
\emph{UP: what is a perceptual front-end? you haven't told me as a reader yet.}
and we now have an interface for combining that with relational reasoning modules we can develop and evaluate neural modules for complex relational reasoning in isolation.
As such, we propose to evaluate relational reasoning modules on a host of known problems requiring complex relational reasoning. Predicting long-range consequences of moves in all kinds of games; chess, backgammon, Go, card games, etc. Solving cross-word puzzles, murder mysteries, Sudoku's, 8 queens, graph coloring problems, satisfiability problems, assignment and routing problems, constraint satisfaction problems etc.

\emph{UP. here, you have to enumerate things that are close you your results. if you mention chess and spread the net too wide, you give reviewers ammunition to criticize your approach.}

In this paper we consider the problem of solving 9x9 Sudokus with as little as 17 givens, which requires an order of magnitude more reasoning steps than BaBi or CLEVR. To solve this challenging task we propose the Recurrent Relational Network (RRN), a graph neural network for solving problems that require complex relational reasoning. It can be added to any deep model that requires complex relational reasoning.

\emph{UP. This task doesn't seem to use messy, noisy censors...?}

We evaluate the RRN on the 9x9 Sudoku problem where it solves 96.6\% of puzzles with the minimum of 17 givens. For more givens the accuracy quickly approaches 100\%. The RRN learns a convergent message passing inference algorithm that outperforms the traditional sum product message passing algorithm.
The non-recurrent relational network cannot solve even simple Sudoku's with 34 givens, as multiple steps of relational inference is required. To compare our model to others we also evaluate the RRN on the more traditional BaBi dataset solving 19/20 tasks, which is competitive with state-of-the-art Sparse Differential Neural Computers.

\emph{UP. this (above) is a key part of your sales pitch, and the example should be folded in earlier, even as PROBLEM A.}


==> ulrich-2.tex <==
%%%%%%%%
% Some shortcuts to simplify all the math.
\def\argmax{\operatornamewithlimits{arg\,max}}
\def\argmin{\operatornamewithlimits{arg\,min}}

\DeclareMathOperator{\sigmoid}{sigm}

\def\const{\mathsf{const}}
\def\data{\mathsf{data}}
\def\det{\mathsf{det}}
\def\diag{\mathsf{diag}}
\def\latest{\mathsf{latest}}
\def\linear{\mathsf{lin}}
\def\nnet{\mathrm{nnet}}
\def\nonlin{\mathsf{f}}
\def\nrelu{\mathsf{nrelu}}
\def\old{\mathsf{old}}
\def\relu{\mathsf{relu}}
\def\sigmoid{\mathrm{sigm}}
\def\slab{\mathsf{sslab}}
\def\slice{\mathsf{slice}}
\def\srelu{\mathsf{srelu}}
\def\trace{\mathsf{tr}}
\def\unif{\mathsf{unif}}
\def\var{\mathsf{var}}
\def\wo{\backslash}

\def\a{\mathbf{a}}
\def\b{\mathbf{b}}
\def\c{\mathbf{c}}
\def\e{\mathbf{e}}
\def\f{\mathbf{f}}
\def\g{\mathbf{g}}
\def\h{\mathbf{h}}
\def\i{\mathbf{i}}
\def\m{\mathbf{m}}
\def\o{\mathbf{o}}
\def\r{\mathbf{r}}
\def\s{\mathbf{s}}
\def\u{\mathbf{u}}
\def\v{\mathbf{v}}
\def\w{\mathbf{w}}
\def\x{\mathbf{x}}
\def\y{\mathbf{y}}
\def\z{\mathbf{z}}

\def\0{\mathbf{0}}
\def\1{\mathbf{1}}
\def\2{\mathbf{2}}
\def\A{\mathbf{A}}
\def\B{\mathbf{B}}
\def\C{\mathbf{C}}
\def\D{\mathbf{D}}
\def\E{\mathbf{E}}
\def\H{\mathbf{H}}
\def\I{\mathbf{I}}
\def\L{\mathbf{L}}
\def\P{\mathbf{P}}
\def\Q{\mathbf{Q}}
\def\R{\mathbf{R}}
\def\S{\mathbf{S}}
\def\U{\mathbf{U}}
\def\V{\mathbf{V}}
\def\W{\mathbf{W}}
\def\X{\mathbf{X}}
\def\Y{\mathbf{Y}}
\def\Z{\mathbf{Z}}

\def\balpha{\bm{\alpha}}
\def\bbeta{\bm{\beta}}
\def\etab{\bm{\eta}}
\def\bepsilon{\bm{\epsilon}}
\def\bgamma{\bm{\gamma}}
\def\bGamma{\bm{\Gamma}}
\def\blambda{\bm{\lambda}}
\def\bLambda{\bm{\Lambda}}
\def\bmu{\bm{\mu}}
\def\bnu{\bm{\nu}}
\def\bomega{\bm{\omega}}
\def\bOmega{\bm{\Omega}}
\def\bphi{\bm{\phi}}
\def\bpi{\bm{\pi}}
\def\bsigma{\bm{\sigma}}
\def\bSigma{\bm{\Sigma}}
\def\btheta{\bm{\theta}}

\def\drm{\mathrm{d}}
\def\erm{\mathrm{e}}
\def\mrm{\mathrm{m}}

\def\vfrak{\mathfrak{v}}

\def\EP{\mathsf{EP}}
\def\LSTM{\mathsf{LSTM}}
\def\KL{\mathsf{D}_{\mathsf{KL}}}
\def\VB{\mathsf{VB}}

\def\Ebb{\mathbb{E}}
\def\Ibb{\mathbb{I}}
\def\Rbb{\mathbb{R}}
\def\Vbb{\mathbb{V}}

\def\Acal{\mathcal{A}}
\def\Bcal{\mathcal{B}}
\def\Dcal{\mathcal{D}}
\def\Fcal{\mathcal{F}}
\def\Hcal{\mathcal{H}}
\def\Kcal{\mathcal{K}}
\def\Lcal{\mathcal{L}}
\def\Mcal{\mathcal{M}}
\def\Ncal{\mathcal{N}}
\def\Ocal{\mathcal{O}}
\def\Qcal{\mathcal{Q}}
\def\Rcal{\mathcal{R}}
\def\Scal{\mathcal{S}}
\def\Tcal{\mathcal{T}}
\def\Ucal{\mathcal{U}}
\def\Xcal{\mathcal{X}}
\def\Ycal{\mathcal{Y}}
\def\Zcal{\mathcal{Z}}

\def\csf{\mathsf{c}}
\def\fsf{\mathsf{f}}
\def\hsf{\mathsf{h}}
\def\isf{\mathsf{i}}
\def\osf{\mathsf{o}}
\def\usf{\mathsf{u}}
\def\wsf{\mathsf{w}}
\def\ysf{\mathsf{y}}

\def\defined{\stackrel{\text{\tiny def}}{=}}
\def\isitequal{\stackrel{\text{\tiny ?}}{=}}

\newcommand{\comment}[1]{\textcolor{blue}{\it [{#1}]}}
\newcommand{\cleancomment}[1]{\textcolor{blue}{\it {#1}}}
\newcommand{\todo}[1]{\textcolor{blue}{\it {\bf To do:} {#1}}}

\definecolor{Purple}{rgb}{0.63,0.1,0.76}
\definecolor{DarkGreen}{rgb}{0.1,0.7,0.2}
\definecolor{LightGray}{rgb}{0.73,0.7,0.65}

\newcommand{\tblue}[1]{\textcolor{blue}{#1}}
\newcommand{\tpurple}[1]{\textcolor{Purple}{#1}}
\newcommand{\tred}[1]{\textcolor{red}{#1}}
\newcommand{\tgreen}[1]{\textcolor{DarkGreen}{#1}}
\newcommand{\tlightgray}[1]{\textcolor{LightGray}{#1}}
%%%%%%%%

\section{Recurrent Relational Networks}

The reasoning involved in solving tasks like Sudoku has both a recurrent and a relational component: recurrent, as a solution is iteratively refined, and relational, as the different substructures in the problem are intimately related.
In this section, we will use Sudoko as a running, but by no means exclusive, example.
It can be formulated as a graph with $i \in \{1,2, .., I \}$ nodes ($I = 81$), one for each Sudoko cell, with a valid solution $\y \in \{ 1, .., C \}^{81}$, where each $y_i$ takes one of $C = 9$ values.
Each node has an edge to and from all nodes in the same row, column and box in the Sudoku.
Each node has a feature vector $\x_i$, and the feature vectors
$\X \defined \{\x_1, .., \x_{I}\}$ serve as input for relational reasoning.
\emph{I'm not clear what they are. Details. ``For our Sudoku example each $x_i$ encodes the initial cell content and the row and column position.'' means?}
More generally, outside the Sudoko running example, features $\X$ could arise from a function or transformation of any other input,
like an audio-visual stream.

To perform recurrent relational reasoning, we associate a hidden state
$\h_i^t$ with every node $i$ at time step $t$, such that
$\H^t \defined \{ \h_i^t\}_{i=1}^{I}$ defines the collection of hidden states in the graph. We assume that relational reasoning will proceed for $T$ steps,
and refine the predictions for a valid solution $\y$ from $\X$ and
$\h_i^0 = \0$ over $T$ attempts on $T$ copies of $\y$:
%%
\begin{equation}
\label{eq:objective}
p( \{ \y \}_{t=1}^T | \X; \H^0) = \prod_{t=1}^T p(\y | \X; \H^t) \ .
\end{equation}
%%
The individual predictive probabilities are Bernoulli, and are detailed in Eq.~(TO COME LATER).
The representation leading to a solution is refined by propagating information through the graph, by letting
the hidden states for all the nodes $i$ in the graph temporally depend on their preceding states through a composite function,
%%
\begin{equation}
\label{eq:recurrent}
\h_{i}^{t+1} =
g \left( \h_i^{t}, \sum_{j \in N(i)} f( \h_i^{t}, \h_j^{t}), \, \x_i \right) \ .
\end{equation}
%%
The function $g$ is, for instance, an \emph{LIST OF EXAMPLES HERE}, and takes as input node $i$'s feature $\x_i$ and state $\h_i^t$ at time $t$.
It furthermore relies on learned relational information coming from node $i$'s neighbors $j \in N(i)$. The relational information takes the form of
incoming messages
\[
\m_{ij}^t \defined f( \h_i^{t}, \h_j^{t}) \ ,
\]
which are summed together in \eqref{eq:recurrent}.
The function $f$ that combines the information from neighboring states is a \emph{WHAT IS IT?}.
In the case of Sudoku, these messages implement an
elimination strategy at convergence, slowly incorporating relational information to downweight implausible predictions for $\y$.
This is illustrated in Sec.~{REF} in the results.

Now that the recurrent connections updates between states in the relational graph are defined, we turn again to the objective function in \eqref{eq:objective}, which, for the Sudoku example, we model as a product of Bernoulli observations,
\[
p( \{ \y \}_{t=1}^T | \X; \H^0) = \prod_{t=1}^T \prod_{i=1}^{I} \textrm{Ber} \left(y_i ; \frac{\erm^{r_{y_i}(\h_i^t)}}{\sum_{c=1}^C \erm^{r_c(\h_i^t)}} \right) \ .
\]
The logits $r(\h_i^t) \in \Rbb^C$ in the Bernoulli odds are parameterized
by a function $r$ that \emph{DETAILS ABOUT WHAT IT DOES.}
